Convexity and Order in Probabilistic Call-by-Name FPC

Kegelspitzen are mathematical structures coined by Keimel and Plotkin, in order to encompass the structure of a convex set and the structure of a dcpo. In this paper, we ask ourselves what are Kegelspitzen the model of. We adopt a categorical viewpoint and show that Kegelspitzen model stochastic matrices onto a category of domains. Consequently, Kegelspitzen form a denotational model of pPCF, an abstract functional programming language for probabilistic computing. We conclude the present work with a discussion of the interpretation of (probabilistic) recursive types, which are types for entities which might contain other entities of the same type, such as lists and trees.

==> notations.tex <==
% Configuration des théorèmes

%\newtheorem{mytheo}{Theorem}[section]
%\newtheorem{myprop}[mytheo]{Proposition}
%\newtheorem{mycoro}[mytheo]{Corollary}
%\newtheorem{mylem}[mytheo]{Lemma}
%
%\theoremstyle{definition}
%\newtheorem{mydef}[mytheo]{Definition}
%
%\theoremstyle{remark}
%\newtheorem{mynot}[mytheo]{Notation}
%\newtheorem{mysam}[mytheo]{Example}
%\newtheorem{myrem}[mytheo]{Remark}
%\newtheorem{myprob}[mytheo]{Open problem}

%\everymath=\expandafter{\the\everymath\displaystyle}

\newcommand{\op}[1]{\textsf{#1}}

%Commandes mathématiques
\newcommand{\bra}[1]{\left\langle #1 \right|}
\newcommand{\ket}[1]{\left| #1 \right\rangle}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\demi}{\frac{1}{2}}
\newcommand{\IC}{\textsc{I}}
\newcommand{\vect}[1]{\overrightaErrow{#1}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\PX}{\mathcal{P}(X)}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\deriv}{\mathrm{d}}
\newcommand{\prodscal}[2]{\left\langle #1 \vert #2 \right\rangle}
\newcommand{\scprod}{\mathrel{\bullet}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\set}[1]{\left\lbrace #1 \right\rbrace}
\newcommand{\pair}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\ltwo}{\ell^2}
\newcommand{\unit}{[0,1]}
\newcommand{\linspan}{\operatorname{span}}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
\newcommand{\kl}[1]{{\mathcal Kl}(#1)}
\newcommand{\kln}[1]{{\mathcal Kl_{\N}}(#1)}
\newcommand{\EiMo}{\mathcal{EM}}
\newcommand{\Ef}{\operatorname{Ef}}
\newcommand{\lwnr}{\sqsubseteq}
\newcommand{\fix}{\operatorname{fix}}
\newcommand{\dirsubset}{\subseteq_{dir}}
\newcommand{\lub}{\bigvee}
\newcommand{\glb}{\bigwedge}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\wkp}{\operatorname{wp}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\trn}{\tr_n}
\newcommand{\nattrans}{\Rightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\supp}{\operatorname{supp}}

\newcommand{\lublambda}{\lub_{\lambda}}
\newcommand{\lubgamma}{\lub_{\gamma}}

\newcommand{\cat}[1]{\mathbf{#1}}
\newcommand{\Conv}{\mathbf{Conv}}
\newcommand{\SConv}{{\Conv_{\leq 1}}}
\newcommand{\Dcpo}{\mathbf{Dcpo}}
\newcommand{\DcpoS}{\Dcpo_{\perp !}}

\newcommand{\DM}{\mathcal D_{= 1}}
\newcommand{\SDM}{\mathcal D_{\leq 1}}
\newcommand{\DMinf}{\DM^\infty}
\newcommand{\SDMinf}{\SDM^\infty}
\newcommand{\RM}{\mathcal R_{= 1}}
\newcommand{\SRM}{\mathcal R_{\leq 1}}
\newcommand{\EM}{\mathcal E_{= 1}}
\newcommand{\SEM}{\mathcal E_{\leq 1}}
\newcommand{\EA}{\mathbf{EA}}
\newcommand{\EAS}{\EA_{\leq 1}}
\newcommand{\EMod}{\mathbf{EMod}}
\newcommand{\EModS}{\EMod_{\leq 1}}
\newcommand{\GEA}{\mathbf{GEA}}
\newcommand{\GEMod}{\mathbf{GEMod}}
\newcommand{\hyperstonean}{\mathcal{HS}}
\newcommand{\dEMod}{\mathbf{dEMod}}
\newcommand{\dGEMod}{\mathbf{dGEMod}}
\newcommand{\Cone}{\cat{Cone}}
\newcommand{\dCone}{\cat{dCone}}

\newcommand{\dConv}{\cat{d}\Conv}
\newcommand{\dSConv}{\cat{d}\SConv}
\newcommand{\hsEMod}{\hyperstonean\EMod}
\newcommand{\hsGEMod}{\hyperstonean\GEMod}
\newcommand{\QD}{{\mathbf{QD}_{\mathbf{\leq 1}}}}
\newcommand{\QDU}{{\mathbf{QD}_{\mathbf{= 1}}}}

\newcommand{\Fd}{\mathbf{Fd}}
\newcommand{\FdHilb}{\mathbf{FdHilb}}
\newcommand{\WStar}{\mathbf{W^*\text{-}Alg}}
\newcommand{\CStar}{\mathbf{C^*\text{-}Alg}}
\newcommand{\PU}{\CStar_\mathrm{PU}}
\newcommand{\PSU}{\CStar_\mathrm{PSU}}
\newcommand{\PNU}{\CStar_\mathrm{P}}
\newcommand{\CPNU}{\CStar_\mathrm{CP}}
\newcommand{\CPU}{\CStar_\mathrm{CPU}}
\newcommand{\FdCPU}{\Fd\CStar_\mathrm{CPU}}
\newcommand{\CPSU}{\Fd\CStar_\mathrm{CPSU}}
\newcommand{\MIU}{\CStar_\mathrm{MIU}}
\newcommand{\wMIU}{\WStar_\mathrm{MIU}}
\newcommand{\wPU}{\WStar_\mathrm{PU}}
\newcommand{\wPSU}{\WStar_\mathrm{PSU}}
\newcommand{\wCPSU}{\WStar_\mathrm{CPSU}}
\newcommand{\wCPU}{\WStar_\mathrm{CPU}}
\newcommand{\wPNU}{\WStar_\mathrm{P}}
\newcommand{\wCPNU}{\WStar_\mathrm{CP}}
\newcommand{\wNMIU}{\WStar_\mathrm{NMIU}}
\newcommand{\NS}{\mathcal{NS}}
\newcommand{\NSS}{\NS_{\leq 1}}
\newcommand{\KHaus}{\cat{CH}}

\newcommand{\CPM}{\cat{CPM}}
\newcommand{\CPMs}{\cat{CPMs}}
\newcommand{\Q}{\cat{Q}}
\newcommand{\Qubits}{\cat{Qubit_s}}
\newcommand{\Qubit}{\cat{Qubit}}
\newcommand{\QUBIT}{\cat{QUBIT}}
\newcommand{\SConvCpo}{\SConv\Dcpo}
\newcommand{\ConvCpoS}{\Conv\DcpoS}
%\newcommand{\ConvCpo}{\Conv\Dcpo}
%\newcommand{\SConvCpoS}{\SConv\DcpoS}
\newcommand{\ConvCpo}{\dConv}
\newcommand{\SConvCpoS}{\dSConv}
\newcommand{\Clifford}{\cat{Clifford_1}}

\newcommand{\Pred}{\operatorname{Pred}}
\newcommand{\Rel}{\cat{Rel}}
\newcommand{\CEff}{\cat{CEff}}
\newcommand{\CEffRel}{\CEff\Rel}

\newcommand{\opp}[1]{#1^\mathbf{op}}
%\newcommand{\sa}[1]{#1_{\mathrm{sa}}}
\newcommand{\eppair}[2]{\left\langle #1,  #2 \right\rangle}
\newcommand{\id}{\operatorname{id}}
\newcommand{\weakpred}{\operatorname{wp}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\tensor}{\overline{\otimes}}
\newcommand{\bigtensor}{\overline{\bigotimes}}
\newcommand{\guillemets}[1]{\og #1 \fg{}}
\newcommand{\supernote}[1]{$^\text{#1}$}
\newcommand{\supercite}[1]{\supernote{\cite{#1}}}

\newcommand{\new}{\op{new}}
\newcommand{\meas}{\op{meas}}

\newcommand{\QPredom}{\cat{QPredom}}
\newcommand{\QDom}{\cat{QDom}}
\newcommand{\QDomS}{\QDom_!}
\newcommand{\Split}{\cat{Split}}

\newcommand{\todo}[1]{\textbf{TODO: #1}}
\newcommand{\hide}[1]{}

\newcommand{\qubit}{\op{qubit}}
\newcommand{\opunit}{\op{unit}}
\newcommand{\rec}{\op{rec}}
\newcommand{\thunk}{\op{thunk}}
\newcommand{\force}{\op{force}}
\newcommand{\bool}{\op{bool}}
\newcommand{\mat}[1]{M_{#1}}
\newcommand{\FinHilb}{\mathbf{FHilb}}
\newcommand{\Mat}{\mathbb{N}_\mathrm{Mat}}
\newcommand{\Isom}{\mathbb{N}_\mathrm{Isom}}
\newcommand{\NatCP}{\mathbb{N}_\mathrm{CP}}
\newcommand{\NatCPoptU}{\mathbb{N}_\mathrm{CP(U)}}
\newcommand{\NatCPU}{\mathbb{N}_\mathrm{CPU}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\myparagraph}[1]{\noindent\textit{#1.}}

\newcommand{\myvec}{\pol}

\newcommand{\KS}{\mathbf{KS}}

%New commands related to denotational semantics
\newcommand{\denot}[1]{[\![#1]\!]}
\newcommand{\arrow}{\Rightarrow}

%New commands related to PPCF
\newcommand{\nat}{{\op{nat}}}
\newcommand{\pop}{\op{\texttt{p}}}
\newcommand{\sop}{\op{\texttt{s}}}
\newcommand{\num}[1]{\underline{#1}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\xprobred}[1]{\xrightarrow{#1}}
\newcommand{\probred}{\xprobred{\kappa}}
\newcommand{\detred}{\to_d}
\newcommand{\ifop}{\op{if}}
\newcommand{\fixop}{\op{fix}}
\newcommand{\Prob}{\op{Prob}}
\newcommand{\PCS}{\cat{PCS}}

%New commands related to PPCFu
\newcommand{\undef}{\operatorname{\mathtt{undef}}}
\newcommand{\PPCFu}{PPCF$_\perp$}

%New commands related to QPCF
\newcommand{\true}{\op{true}}
\newcommand{\false}{\op{false}}
\newcommand{\qtrue}{\op{qtrue}}
\newcommand{\qfalse}{\op{qfalse}}
\newcommand{\xqrand}[1]{\op{qrand}(#1)}
\newcommand{\qrand}{\xqrand{\lambda}}
\newcommand{\bit}{\op{bit}}
\newcommand{\xrand}[1]{\op{rand}(#1)}
\newcommand{\rand}{\xrand{\kappa}}
\newcommand{\ketplus}{\ket{+}}
\newcommand{\ketminus}{\ket{-}}
\newcommand{\xqured}[1]{\xrightarrow{\ket{#1}}}
\newcommand{\quredzero}{\xqured{0}}
\newcommand{\quredone}{\xqured{1}}
\newcommand{\quredplus}{\xqured{+}}

\newcommand{\newop}{\op{new}}
\newcommand{\applyop}[1]{\mathtt{#1}}
\newcommand{\applyU}{\applyop{U}}
\newcommand{\measop}{\op{measure}}

\newcommand{\krarr}{\rightsquigarrow}

